SAM-IQA: Can Segment Anything Boost Image Quality Assessment?

Image Quality Assessment (IQA) is a challenging task that requires training on massive datasets to achieve accurate predictions. However, due to the lack of IQA data, deep learning-based IQA methods typically rely on pre-trained networks trained on massive datasets as feature extractors to enhance their generalization ability, such as the ResNet network trained on ImageNet. In this paper, we utilize the encoder of Segment Anything, a recently proposed segmentation model trained on a massive dataset, for high-level semantic feature extraction. Most IQA methods are limited to extracting spatial-domain features, while frequency-domain features have been shown to better represent noise and blur. Therefore, we leverage both spatial-domain and frequency-domain features by applying Fourier and standard convolutions on the extracted features, respectively. Extensive experiments are conducted to demonstrate the effectiveness of all the proposed components, and results show that our approach outperforms the state-of-the-art (SOTA) in four representative datasets, both qualitatively and quantitatively. Our experiments confirm the powerful feature extraction capabilities of Segment Anything and highlight the value of combining spatial-domain and frequency-domain features in IQA tasks. Code: https://github.com/Hedlen/SAM-IQA

==> include/pipeline.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{figs/main_pipeline1.pdf}
\caption{The multi-stage feature distillation pipeline of our method. } \label{rep_megSR}
\end{figure*}


==> include/tab_basline_compare.tex <==
\begin{table*}[]
\centering
\setlength{\tabcolsep}{1.2mm}{
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{Scale} & \multirow{2}{*}{Model}   & Params                & Set5                               & Set14                              & BSD100                             & UrBan100                           & Manga109                           \\
                       &                          &  (M)                        & PSNR/SSIM                          & PSNR/SSIM                          & PSNR/SSIM                          & PSNR/SSIM                          & PSNR/SSIM                          \\ \hline
\multirow{14}{*}{$\times$2}   & SRCNN~\cite{simonyan2014very}                    & 0.024                       & 36.66 / 0.9542                      & 32.42 / 0.9063                     & 31.36 / 0.8879                     & 29.50 / 0.8946                     & 35.60 / 0.9663                       \\
                       & FSRCNN~\cite{dong2016accelerating}                   & 0.012                       & 36.98 / 0.9556                     & 32.62 / 0.9087                     & 31.50 / 0.8904                     & 29.85 / 0.9009                     & 36.67 / 0.9710                       \\
                       & VDSR~\cite{kim2016accurate}                     & 0.666                      & 37.53 / 0.9587                     & 33.05 / 0.9127                     & 31.90 / 0.8960                     & 30.77 / 0.9141                     & 37.22 / 0.9750                       \\    
                       & DRCN~\cite{kim2016deeply}                     & 1.774                     & 37.63 / 0.9588                     & 33.04 / 0.9118                     & 31.85 / 0.8942                     & 30.75 / 0.9133                     & 37.55 / 0.9732                       \\
                       & LapSRN~\cite{lai2017deep}                   & 0.251                      & 37.52 / 0.9591                     & 32.99 / 0.9124                     & 31.80 / 0.8952                     & 30.41 / 0.9103                     & 37.27 / 0.9740                     \\
                       & IDN~\cite{hui2018fast}                      & 0.579                      & 37.83 / 0.9600                     & 33.30 / 0.9148                     & 32.08 / 0.8985                     & 31.27 / 0.9196                     & 38.01 / 0.9749                     \\
                       & EDSR~\cite{lim2017enhanced}                     & 1.370                     & 37.91 / 0.9602                     & 33.53 / 0.9172                     & 32.15 / 0.8995                     & 31.99 / 0.9270                     & 38.40 / 0.9766                     \\
                       & CARN~\cite{ahn2018fast}                     & 1.592                     & 37.76 / 0.9590                     & 33.52 / 0.9166                     & 32.09 / 0.8978                     & 31.92 / 0.9256                     & 38.36 / 0.9765                     \\
                       
                       & ECBSR~\cite{zhang2021edge}                    & 0.596                      & 37.90 / \textcolor{red}{0.9615}                     & 33.34 / 0.9178                     & 32.10 / \textcolor{red}{0.9018}                     & 31.71 / 0.9250                     & - / -                                \\
                       & IMDN~\cite{hui2019lightweight}                     & 0.694                      & \textcolor{blue}{38.00} / 0.9605                     & 33.63 / 0.9177                     & \textcolor{blue}{32.19} / 0.8996                     & \textcolor{blue}{32.17} / \textcolor{blue}{0.9283}                     & \textcolor{red}{38.88} / \textcolor{red}{0.9774}                     \\
                       & RFDN~\cite{liu2020residual}                     & 0.534                      & \textcolor{red}{38.05} / \textcolor{blue}{0.9606}                     & \textcolor{red}{33.68} / \textcolor{blue}{0.9184}                     & 32.16 / 0.8994                     & 32.12 / 0.9278                     & \textcolor{blue}{38.88} / \textcolor{blue}{0.9773}                     \\
                       & Ours                     & 0.527                      & 37.98 / 0.9605                       & \textcolor{blue}{33.66} / \textcolor{red}{0.9192}                       & \textcolor{red}{32.20} / \textcolor{blue}{0.9002}                       & \textcolor{red}{32.31} / \textcolor{red}{0.9302}                       & 38.62 / 0.9770                       \\ \hline
\multirow{14}{*}{$\times$4}   & SRCNN~\cite{simonyan2014very}                    & 0.057                       & 30.48 / 0.8628                       & 27.49 / 0.7503                       & 26.90 / 0.7101                       & 24.52 / 0.7221                     & 27.58 / 0.8555                       \\
                       & FSRCNN~\cite{dong2016accelerating}                   & 0.013                       & 30.72 / 0.8660                       & 27.61 / 0.7550                       & 26.98 / 0.7150                       & 24.62 / 0.7280                     & 27.90 / 0.8610                       \\
                       & VDSR~\cite{kim2016accurate}                      & 0.666                      & 31.35 / 0.8838                       & 28.01 / 0.7674                       & 27.29 / 0.7251                       & 25.18 / 0.7524                     & 28.83 / 0.8870                       \\
                       & DRCN~\cite{kim2016deeply}                     & 1.774                     & 31.53 / 0.8854                       & 28.02 / 0.7670                       & 27.23 / 0.7233                       & 25.14 / 0.7510                     & 28.93 / 0.8854                       \\
                       & LapSRN~\cite{lai2017deep}                   & 0.502                      & 31.54 / 0.8852                       & 28.09 / 0.7700                       & 27.32 / 0.7275                       & 25.21 / 0.7562                     & 29.09 / 0.8900   \\
                       & IDN~\cite{hui2018fast}   & 0.600  & 31.93 / 0.8923 & 28.45 / 0.7781 & 27.48 / 0.7326 & 25.81 / 0.7766 & 30.04 / 0.9026 \\
                       &  EDSR~\cite{lim2017enhanced} & 1.518 & 31.98 / 0.8927 & 28.55 / 0.7805 & 27.54 / 0.7348 & 25.90 / 0.7809 & 30.24 / 0.9053 \\
                       & CARN~\cite{ahn2018fast}                     & 1.592                     & 32.13 / 0.8937                       & \textcolor{blue}{28.60} / 0.7806                       & \textcolor{blue}{27.58} / 0.7349                       & 26.07 / 0.7837                     & 30.47 / 0.9084                     \\

                       & ECBSR~\cite{zhang2021edge}                     & 0.603                      & 31.92 / 0.8946                       & 28.34 / \textcolor{blue}{0.7817}                       & 27.48 / \textcolor{red}{0.7393}                       & 25.81 
 / 0.7773                      & - / -                                \\
                       & IMDN~\cite{hui2019lightweight}                     & 0.715                      & \textcolor{blue}{32.21} / 0.8948                       & 28.58 / 0.7811                       & 27.56 / 0.7353                       & 26.04 / 0.7838                     & 30.45 / 0.9075 \\
                       & RFDN~\cite{liu2020residual}                     & 0.550                      & \textcolor{red}{32.24} / \textcolor{red}{0.8952}                      & \textcolor{red}{28.61} / \textcolor{red}{0.7819}                       & 27.57 / 0.7360                       & \textcolor{blue}{26.11} / \textcolor{blue}{0.7858}                     & \textcolor{red}{30.58} / \textcolor{red}{0.9089}                     \\
                       & Ours                     & 0.543                      & 32.20 / \textcolor{blue}{0.8950}                       & 28.58 / 0.7811                       & \textcolor{red}{27.59} / \textcolor{blue}{0.7364}                       & \textcolor{red}{26.16} / \textcolor{red}{0.7879}                       & \textcolor{blue}{30.53} / \textcolor{blue}{0.9087}                       \\ \hline
\end{tabular}}
\caption{Quantitative results of the state-of-the-art efficient super-resolution models on four benchmark datasets. The best and second-best results are marked in \textcolor{red}{red} and  \textcolor{blue}{blue} colors, respectively.}
\label{tab:quantitative}
\end{table*}


  

==> include/teaser.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figs/teaser3.pdf}
\caption{Comparison with recent efficient SR methods. The figure shows the GFLOPs of these methods when the input is 256\(\times\)256, the number of parameters of these models and their average inference time using NVIDIA 2080ti under the DIV2K validation set.} \label{fig:teaser}
\end{figure}


